Polynomial Convergence of Bandit No-Regret Dynamics in Congestion Games

We introduce an online learning algorithm in the bandit feedback model that, once adopted by all agents of a congestion game, results in game-dynamics that converge to an $\epsilon$-approximate Nash Equilibrium in a polynomial number of rounds with respect to $1/\epsilon$, the number of players and the number of available resources. The proposed algorithm also guarantees sublinear regret to any agent adopting it. As a result, our work answers an open question from arXiv:2206.01880 and extends the recent results of arXiv:2306.15543 to the bandit feedback model. We additionally establish that our online learning algorithm can be implemented in polynomial time for the important special case of Network Congestion Games on Directed Acyclic Graphs (DAG) by constructing an exact $1$-barycentric spanner for DAGs.

==> sections/bandit-alg.tex <==
In this section we present our proposed no-regret algorithm for general congestion games that once adopted by all agents, convergence to NE is achieved. Before presenting our algorithm we present some preliminary definitions common in the bandits and optimization literature.



\subsection{Our Algorithms and Guarantees}

We are ready to present our proposed algorithm for general congestion games. It is given in Algorithm~\ref{alg:bandit-alg}. The main technical results verified by this scheme are detailed in what follows. The no-regret result (Theorem \ref{thm:bigRegret}) is a corollary of the following theorem.


\begin{restatable}[Sublinear Regret]{theorem}{subregret}
\label{thm:sublin}
    Let $i \in [n]$. Let $p_i^{1:T}$ be the sequences of strategies produced by \texttt{Algorithm}~\ref{alg:bandit-alg} for the sequence of costs $c^{1:T}$. Let $u \in \calS_i$. We have with probability $1-\delta$,
    \[
        \Regret\br{p_i^{1:T}, c^{1:T}; u} \leq \tilde{O}\br{ \frac{m}{\gamma_T} + \sum_{t=1}^{T}\br{\vartheta^2m^6 c^2_{\max}\frac{\gamma_t}{\mu_t^2} + mc_{\max}\mu_t} + \sqrt{\sum_{t=1}^{T}\frac{\vartheta^{3}m^{6}c^2_{\max}}{\mu_t^2}} + mc_{\max}\sqrt{T}}.
    \]
\end{restatable}

The accompanying result on convergence to equilibrium \ref{thm:bigNash} is a corollary of the following theorem.

\begin{theorem}[Convergence to Nash] 
\label{thm:smallNash}
Let all agents adopt Algorithm~\ref{alg:bandit-alg}. Let $\epsilon > 0$ and $\pi^1, \dots, \pi^T$ denote the sequence of joint strategy profiles produced. Let $t$ be uniformly sampled from $[T]$. For any $\delta \in (0, 1)$, the joint strategy $\pi_t$ is a 
\[
\frac{1}{L_{\Phi}\delta}\br{\sqrt{\frac{\Phi_{\max} + L_{\Phi}nm}{T\gamma_T} + \frac{1}{T\gamma_T} \sum_{t=1}^{T}\br{nmL_{\Phi}^2\gamma_t\mu_t + \vartheta^2m^6c_{\max}\frac{\gamma_t^2}{\mu^2_t}}} + nmc_{\max}\frac{1}{T}\sum_{t=1}^T\mu_t}-\text{mixed-Nash equilibrium},
\]
with probability $(1-\delta)$.

\end{theorem}

We provide detailed proof sketches in section \ref{sec:sketches} and defer the complete proofs to the appendix.



==> sections/basis.tex <==
For a given agent $i$, we denote by $\calS_i \subset \R^m$, the strategy space corresponding to set of all paths connecting $s_i$ to $t_i$. We can restrict our attention to the subgraph $G_i = (V_i, E_i)$ where $V_i$ and $E_i$ corresponds to the nodes and edges appearing in at least one path in $\calS_i$.

\subsection{Blue edges}

The convex hull of the strategy space $\calS_i$ forms the path polytope $\calX_i = \text{conv}(\calS_i)$. This polytope is included in a subspace of $\R^{m}$ of dimension $m_i - n_i + 2$, where $n_i = |V_i|$. Indeed, for each node $v \in V \backslash \{s_i, t_i\}$, we can pick one outgoing edge $e_v^* \in \text{out}(v)$ such that for any $x \in \calP_i$, we have
\begin{equation}
\label{eq:predictable}
x_{e_v^*} = \sum_{e \in \text{in}(v)} x_e - \sum_{e \in \text{out}(v), e \neq e_v^* } x_e
\end{equation}
for all $v \in V \backslash \{s_i, t_i\}$. These equations come from reasoning about flow preservation.
Consequently, $\calX_i$ belongs to the intersection of $n_i - 2$ hyperplanes, which is of dimension at most $m_i - n_i + 2$. In other words, although the strategy space is of dimension $m_i$, the degrees of freedom are restricted by the graph structure as some coordinates are redundant and predictable from other coordinates (see \eqref{eq:predictable}). We single out these redundant edges in the following definition.

\begin{definition}
For all $v \in V_i \backslash \{s_i, t_i\}$ (i.e all nodes except the blueting and termination nodes), we arbitrarily pick one edge denoted $e_v^* \in \text{out}(v)$ that will be referred to as a \textit{{\textcolor{blue}{blue}} edge}.
\end{definition}

The remaining edges will be referred to as a \textcolor{red}{red} edges. These red edges will aid us in constructing a $1$-spanner. Indeed, from equation \eqref{eq:predictable}, we can see that the coordinates corresponding to \textcolor{blue}{blue} edges can be determined by the values at the \textcolor{red}{red} edges.

\subsection{Basis construction}

Let $v_1=s_i, v_2,  \dots, v_n = t_i$ be a topological ordering of the nodes of $G_i$. This induces a topological ordering on the edges (sorted according to their origin node). We will construct a $1$-spanner for $\calX_i$ following this ordering. The following simple lemma about blue paths will be essential.

\begin{definition}[Blue path]
    A path in $G_i$ is said to be a \emph{blue path} if consists entirely of blue edges.
\end{definition}

\begin{lemma}[Blue path lemma]
\label{lem:clean-path}
For any node $v_k \in V_i \backslash \{s_i\}$, there exists a blue path connecting $v_k$ to $v_n = t_i$.
\end{lemma}
\begin{proof}
We proceed by induction on the topological ordering.
For $v_{n-1}$, we pick a blue outgoing  edge. By definition of a topological ordering, the chosen edge will necessarily lead to $v_n = t_i$.

Now let $k \in [2, n-2]$ and assume that the lemma holds for all for $l > k$. We consider the node $v_{k}$ and pick an outgoing blue edge. It will lead to a node $v_l$ with $l > k$. By induction hypothesis, there exists a path connecting $v_l$ to $t_i$ that only consists of blue edges. Concatenating the picked outgoing edge with this path yields the result for $v_k$ so the lemma holds for $k$.
\end{proof}

We can now begin our recursive construction of our basis $b_1, \dots, b_s$ where $s = m_i - n_i + 2$ is the total number of red edges. 

\begin{algorithm}[h]
			\caption{Edge covering basis}
			\label{alg:basis}
			\begin{algorithmic}[1]
				\STATE {\bfseries Input:} Red edges $e_1, \dots, e_s$ in topological order.
                  \smallskip
                  \STATE $\mathrm{Basis} \leftarrow \varnothing$
                  \FOR{$h=1$ to $s$}
                    \STATE Let Blue$(e_h, t_i)$ be the \textit{blue path} connecting $\text{dest}(e_h)$ to $t_i$ (given by Lemma \ref{lem:clean-path}).
                    \FOR{$k=h-1$ to $1$}
                    \IF{ there exists a path $p_{k\rightarrow h}$ joining $\text{dest}(e_k)$ to $\text{source}(e_h)$}
                        \STATE Set $b_h \gets$ Truncate$(b_k, e_k)\;|\;p_{k\rightarrow h}\;|\; p_{e_h \rightarrow t_i}$
                        \STATE Set \texttt{Prefix}$(h) \gets k$  \textcolor{red}{break the for loop if we entered the if ?}
                    \ENDIF
                    \ENDFOR
                    \IF{there is no preceding red edge connected to $e_h$}
                    \STATE Set $b_h \gets$ Blue$(s_i, e_h)\;|\; p_{e_h \rightarrow t_i}$
                    \STATE Set \texttt{Prefix}$(h) \gets \bot$
                    \ENDIF
                    \STATE $\mathrm{Basis} \leftarrow \mathrm{Basis} \cup \{ b_h \}$ 
                  \ENDFOR
				\STATE {\bfseries return} $\mathrm{Basis}$
			\end{algorithmic}
\end{algorithm}


\begin{proposition}[Prefix property]
Consider a covering basis generated by Algorithm~\ref{alg:basis}. Let $e_k < e_l$ be two red edges. If $e_k$ and $e_l$ are connected in $G(V_i, E_i)$, then 
\texttt{Prefix}$(k) \neq\texttt{Prefix}(l)$ where \texttt{Prefix} is the value set at lines $8$ and $13$.
\label{prop:prefix} 
\end{proposition}
\begin{proof}
    Suppose $i = \texttt{Prefix}(k) = \texttt{Prefix}(l)$. Then by construction $e_i<e_k<e_l$. On the other hand, since the prefixes are set in reverse topological order and $e_k$ and $e_l$ are connected, we must have \texttt{Prefix}$(l) \geq k$. A contradiction.
\end{proof}


\begin{theorem}[1-Spanner]
Let $b_1, \dots, b_s$ be the covering basis generated by \texttt{Algorithm}~\eqref{alg:basis}. For any $x \in \calX_i$, there exists $\alpha \in \R^s$ such that
\[
x = \sum_{h=1}^{s} \alpha_h b_i \quad\quad \text{ and } \alpha_h^2 \leq 1
\]
\end{theorem}
\begin{proof}
    It suffices to prove the result for $x \in \calS_i$, the extreme points of $\calX_i$. Let $r_x = \text{Red}(x) \in \R^s$ where $\text{Red}$ is the linear operator selecting the coordinates corresponding to the red edges. Correspondingly, let us define $r_1, \dots, r_s$ such that
    \[
    r_h = \text{Red}(b_h)
    \]
    for $h=1, \dots, s$. Observe that the canonical basis vectors $v_1, \dots, v_s$ of $\R^s$ can be expressed as
    \[
    v_h = r_h - r_{\texttt{Prefix}(h)}
    \]
    for $h=1, \dots, s$, and taking $r_{\bot} = 0_s$. Consequently,
    \[
    r_x = \sum_{h\in r_x} v_h = \sum_{h\in r_x}  \br{r_h - r_{\texttt{Prefix}(h)}} = \sum_{h =1}^{s} \alpha_h r_h
    \]
    for some $\alpha \in \R^s$. Now it remains to prove that $|\alpha_h|\leq 1 $. 

    By the prefix property \ref{prop:prefix}, the mapping $\texttt{Prefix}: \{h: h\in r_x\} \rightarrow [s-1] \cup \{\bot\}$ is injective since the edges in $\{h: h\in r_x\}$ are connected. In other words, there are no duplicates in $\{\texttt{Prefix}(h), h\in r_x\}$.

    Now, let $h \in [s]$,
    \begin{itemize}
        \item If $h \in r_x$, we have that if $h \in \{\texttt{Prefix}(h), h\in r_x\}$, then $\alpha_h = 0$
            otherwise $\alpha_h = 1$.
        \item If $h \notin r_x$, we have that if $h \in \{\texttt{Prefix}(h), h\in r_x\}$, then $\alpha_h = -1$
            otherwise $\alpha_h = 0$.
    \end{itemize}
    We have thus shown that $\alpha_h^2 \leq 1$. Now to conclude, we know from \eqref{eq:predictable} that there exists a linear operator Fill$:\R^s \rightarrow \R^m$ that \textit{fills} in the values of the blue edges from the coordinate values of the red edges, hence $x = \text{Fill}\br{\text{Red}\br{x}}$, which yields,
    \[
    x = \text{Fill}\bs{\sum_{h =1}^{s} \alpha_h r_h} = \sum_{h =1}^{s} \alpha_h \text{Fill}\bs{r_h} = \sum_{h =1}^{s} \alpha_h b_h.
    \]
\end{proof}



%\begin{theorem}[Well separated basis]
%    Let $p_1, \dots, p_s \in \R^m$ be the basis constructed by \texttt{Algorithm} \ref{alg:basis}. It holds that
%    \[
%    \lambda_+ \left(\sum_{i=1}^{s} p_ip_i^\top \right) \geq \frac{1}{{4m}},
%    \]
%    where $\lambda_+$ is the smallest non-zero eigenvalue.
%    \label{thm:separation}
%\end{theorem}

%\begin{lemma}[Coordinate pruning]
%    Let $B \in \R^{s \times m}$ be a selection matrix that drops the coordinates corresponding to blue edges. Let $\tilde{p}_1, \dots, \tilde{p}_s \in \R^s$ be such that $\tilde{p}_k = Bp_k$ for all $k \in [s]$, where $p_1, \dots, p_s$ is the basis constructed by \texttt{Algorithm} \ref{alg:basis} then it holds that
%    \[
%    \lambda_{\min} \left(\sum_{i=1}^{s} \tilde{p}_i\tilde{p}_i^\top \right) \leq \lambda_+ \left(\sum_{i=1}^{s} p_ip_i^\top \right).
%    \]
%\label{lem:pruning}
%\end{lemma}
%\begin{proof}
%    By the min-max theorem (or the Courant-Fisher-Weyl minmax principle), we know that
%    \[
%    \lambda_{\min} \left(\sum_{i=1}^{s} \tilde{p}_i\tilde{p}_i^\top \right)= \min_{\substack{x \in \R^s \\ x\neq 0}} \frac{x^\top \left(\sum_{i=1}^{s} \tilde{p}_i\tilde{p}_i^\top \right) x}{x^\top x}.
%    \]
%    Using the definition of the $\tilde{p}$'s, we have that
%    \[
%    \begin{aligned}
%    \lambda_{\min}\left(\sum_{i=1}^{s} \tilde{p}_i\tilde{p}_i^\top \right) & = \min_{\substack{x \in \R^s \\ x\neq 0}} \frac{x^\top B \left(\sum_{i=1}^{s} {p}_i{p}_i^\top \right) B^\top x}{x^\top x} \\
%    &= \min_{\substack{x \in \R^s \\ x\neq 0}} \frac{x^\top B \left(\sum_{i=1}^{s} {p}_i{p}_i^\top \right) B^\top x}{x^\top BB^\top x} \quad \text{since $BB^\top = I_s$} \\
%    &= \min_{\substack{z \in \R^m \\ z\neq 0 \\ z \in \text{span}(B^\top)}} \frac{z \left(\sum_{i=1}^{s} {p}_i{p}_i^\top \right) z}{z^\top z} \;  \\
%    & \leq \max_{\substack{E \subset \R^m \\ \text{dim}(E) = s}} \min_{\substack{z \in E \\ z\neq 0}} \frac{z \left(\sum_{i=1}^{s} {p}_i{p}_i^\top \right) z}{z^\top z} = \lambda_{m - s + 1} \left(\sum_{i=1}^{s} p_ip_i^\top \right).
%    \end{aligned}
%    \]
%    Moreover, since $p_1, \dots, p_s$ are linearly independent in $\R^m$, $\lambda_{m - s + 1}$ corresponds to the first non-zero eigenvalue.
%\end{proof}

%\begin{lemma}
%    Let $\tilde{p}_1, \dots, \tilde{p}_s \in \R^s$ be defined as in Lemma \ref{lem:pruning}. Because of the prefix property \ref{prop:prefix}, we have that
%    \[
%    \lambda_{\min} \left(\sum_{i=1}^{s} \tilde{p}_i\tilde{p}_i^\top \right) \geq \frac{1}{4s}
%    \]
%\label{lem:polybound}
%\end{lemma}
%\begin{proof}
%We prove the result by induction on the number of red edges $s$.

%For $s=1$, $\tilde{p}^{(s)}_1 = \begin{bmatrix}1\end{bmatrix}$, the result holds.
%Now suppose the result holds for the basis $\tilde{p}^{(s)}_1, \dots, \tilde{p}^{(s)}_s$ generated for $s$ red edges. %When an additional red edge is added, \texttt{Algorithm} \ref{alg:basis} outputs,
%\[
%\tilde{p}^{(s+1)}_k = \begin{bmatrix}\tilde{p}^{(s)}_k & 0 \end{bmatrix} \text{ for } k \in [s] \quad \text{and} \quad %\tilde{p}_{s+1}^{(s+1)} = \begin{bmatrix} \tilde{p}^{(s)}_l & 1 \end{bmatrix} \;\; \text{or}\;\; %\tilde{p}_{s+1}^{(s+1)} = \begin{bmatrix} \mathbf{0}_s & 1 \end{bmatrix}
%\]
%for some $l \leq s$ by the prefix property \ref{prop:prefix}. We can then invoke Theorem \ref{thm:recursivelowerbound} and obtain the result for $s+1$ edges.

%\end{proof}



%A quantity that will play a central role is the first non-zero singular value of $M$. By repeatedly applying the \textit{dependent column lemma}, we can reduce our problem to studying the lower triangular matrix $T$.

%The prefix property will play a central role in proving that the singular value of interest is only polynomially small in $m$.



%First, we observe that the topological ordering of the nodes induces an ordering of the red edges $e_1, \dots, e_s$ as they can be arranged following the order of their source nodes (with an arbitrary ordering if their source nodes coincide). We will cover the edges following this order.

%Let $v_{j_1}$ be the origin of the first red edge $e_1$ and $v_{l_1}$ with $l_1 > j_1$ its destination. By virtue of being the first such node, we can be sure there exists a path $p_{s_i \rightarrow v_{j_1}}$ going from $s_i$ to $v_{j_1}$ that consists only of blue edges. The blue path Lemma \ref{lem:clean-path} ensures there exists a path $p_{v_{l_1} \rightarrow t_i}$ going from $v_{l_1}$ to $t_i$ with only blue edges. We construct the first element of our basis by doing the following concatenation:
%\[
%p_1 = [p_{s_i \rightarrow v_{j_1}} \; | \; e_1 \; | \; p_{v_{l_1} \rightarrow t_i}]
%\]

%Now let $h \in \{1, \dots, s\}$ such that the first $h$ red edges $e_1, \dots, e_h$  have been covered by the paths $p_1, \dots, p_h$. Let us conisder the red edge $e_{h+1}$ and denote $v_{j_{h+1}}$ its origin node and $v_{l_{h+1}}$ its destination. We distinguish two cases. 

%Either there exists a blue path $p_{s_i \rightarrow v_{j_{h+1}}}$ with only blue edges connecting $s_i$ to $v_{j_{h+1}}$. This allows us to construct $p_{h+1}$ with the following concatenation
%\[
%    p_{h+1} = [p_{s_i \rightarrow v_{j_{h+1}}} \; | \; e_{h+1}  \; | \; p_{v_{l_{h+1}} \rightarrow t_i}],
%\]
%where $p_{v_{l_{h+1}} \rightarrow t_i}$ is a blue path with only blue edges whose existence is ensured by Lemma \ref{lem:clean-path}.

%Or $v_{j_{h+1}}$ is only reachable by traversing at least one red edge. Let $p_{s_i \rightarrow v_{j_{h+1}}}$ be such a path, traversing at least one red edge. By virtue of the ordering, the last red edge appearing in $p_{s_i \rightarrow v_{j_{h+1}}}$ must be covered by a path in $p_1, \dots, p_h$. We will denote by $\tilde{p}$ the path covering this last red edge. We observe that we can replace the first portion of $p_{s_i \rightarrow v_{j_{h+1}}}$ from $s_i$ to $v_{j_{h+1}}$ by first following $\tilde{p}$ until the last red edge is traversed, then completing it with the remaining blue edges until $v_{j_{h+1}}$ is reached. With this modification, we proceed with the usual concatenation to construct $p_{h+1}$:
%\[
%p_{h+1} = [p_{s_i \rightarrow v_{j_{h+1}}} \; | \; e_{h+1}  \; | \; p_{v_{l_{h+1}} \rightarrow t_i}]
%\]
%where $p_{v_{l_{h+1}} \rightarrow t_i}$ again comes from \ref{lem:clean-path}.

%This approach progressively covers all the red edges with the paths $p_1, \dots, p_s$. Moreover these paths have the following prefix property which follows immediately from the construction.









==> sections/caratheodory.tex <==
We have constructed a basis for $\calP_i$ in the previous section. We now turn our attention to describing an algorithm for decomposing elements of $\calP_i$ in this basis.

\begin{theorem}
    For any point $x \in \calP^_i$, Algorithm \ref{alg:caratheodory} outputs at most $m$ paths $(\hat{p})_{i=1}^{m} \in \calS_i$ such that 
    \[
    x =  \sum_{k=1}^{m} \lambda_k \hat{p}_k
    \]
    where $\lambda_k \geq 0$ and $\sum_k \lambda_k = 1$.
\end{theorem}


\begin{algorithm}[h]
			\caption{Caratheodory decomposition}
			\label{alg:caratheodory}
			\begin{algorithmic}[1]
				\STATE {\bfseries Input:} A point $x \in \calP^{\mu}_i$
                  \smallskip
                  \STATE $\mathrm{Res} \leftarrow \varnothing$
                \WHILE{$\sum_{e \in \text{out}(s_i)} \tilde{x}_e > 0$}
                    \smallskip
                \STATE $A \leftarrow \{e\in E:~\tilde{x}_e >0\}$
			    \STATE Let $e_{\min} \leftarrow \argmin_{e \in A} x_e$ and $x_{\min} \leftarrow x_{e_{\min}}$.
                \smallskip
			    \STATE $\hat{p} \leftarrow$ An $(s_i, t_i)$-path in $G(V_i, A)$ such that $e_{\text{min}} \in \hat{p}$.
                \smallskip
                \STATE $x_e \leftarrow x_e - x_{\text{min}}$ for all $e \in \hat{p}$.
                \smallskip
                \STATE $\mathrm{Res} \leftarrow \mathrm{Res} \cup \{\left(\hat{p},x_{\text{min}}\right)\}$.
				\ENDWHILE
    
				\STATE {\bfseries return} $\mathrm{Res}$
			\end{algorithmic}
\end{algorithm}


\begin{lemma}
    For any point $x \in \calP_i$, \texttt{Algorithm} \ref{alg:caratheodory} outputs a distribution $\pi \in \Delta(\calS)$ that can be sampled efficiently such that
    \[
    c^\top x = \E_{p \sim \pi}\left[c^\top p\right]
    \]
    for any $c \in \R^m$.
\end{lemma}



==> sections/dags.tex <==
In this section present the algorithm in the special case of network games that runs in polynomial time in terms of $m$ and $n$. 

In network congestion games, we are given a directed acyclic graph $G=(V, E)$, with $m = |E|$. Each agent $i$ has an associated source node $s_i \in V$ and a sink or termination node $t_i \in V$. The set of edges in the graph constitutes the set of ressources in the congestion game. A path connecting a source $s_i$ node to a sink node $t_i$ in $G$ constitutes constitutes a viable strategy for agent $i$. For each agent $i$, we denote by $\calS_i$, the strategy space corresponding to set of all paths connecting $s_i$ to $t_i$. For each agent $i$, we can restrict our attention to the subgraph $G_i = (V_i, E_i)$ where $V_i$ and $E_i$ corresponds to the nodes and edges appearing in at least one path in $\calS_i$.



With the setting of network games fixed, the first step is computing an exploration set that in polynomial-time with respect to the number of resources. The method of \cite{awerbuch2004adaptive} allows one to compute a $\vartheta$-spanner for any $\vartheta > 1$ with a polynomial number of calls to the linear minization oracle over $\calX_i$ after embedding it in a lower dimensional space where it has non empty interior. Instead of adopting their approach, which does not exploit the specific structure of DAGs, we propose an algorithm that stays in the natural parametrization of the problem and outputs a $1$-spanner. The construction is detailed in section \ref{sec:basis} and rests on a clever use of prefix paths. The next theorem follows from that section. 

\begin{theorem}
Given a DAG $G=(V_i, E_i)$ with source $s_i$ and sink $t_i$, there exists a polynomial time algorithm computing an exact $1$-spanner for $\calX_i$.
\end{theorem}

\begin{figure}[h]
    \centering
    \tikz \graph[nodes={draw, circle}, edge quotes={fill=white,inner sep=1pt}] { 
    s -> [thick, red] { b , c [>"first", > bend right, < bend right, <"4"] } -> d -> e -> {f [> thick, > red], g [> bend right, < bend right]} -> t,
    };
    \caption{Construction of a $1$-spanner for DAGs. We can select the three red edges as the basis edges. We cover the edges using 3 paths. For edge $1$, we select $s->b->d->e->g->t$, for edge $2$, we first check if is reachable from edge 1, if not, we find a path starting from $s$. In this case, we select $s->c->d->e->g->t$. For edge $3$ we check if is reachable from the last covered egde(in topological order), we notice it is reachable from edge $2$ so we select $s->c->d->e->f->t$. The key idea we use to construct a 1-spanner is to ensure that when we cover edges, we first try to reach them with the previously covered edges going in reverse topological order. This prefix property ensures the 1-spanner property.}
    \label{fig:basis}
\end{figure}


The second complexity bottleneck is the computation of a Caratheodory decomposition. Fortunately, given a shortest path algorithm, it is possible to compute the decomposition efficiently. The algorithm can be found in \cite{panageas2023semi}. It is a straightforward edge elimination scheme.


==> sections/mirrorNash.tex <==
Let $h: \Delta^{|\calS|} \to \R$ be the negative entropy, i.e, 
\(
h(x) = \sum_{i=1}^m x_i \log(x_i)
\). We define the bregman proximal update $x' = \prox_{\gamma \Phi}(x)$ as
\begin{equation}
x' = \argmin_{z\in \Delta^{|\calS|}} \Phi(Az) + \frac{1}{\gamma}D_h(z, x)
\tag{MD}
\label{eq:MD}
\end{equation}
where $D_h(z, x) = h(z) - h(x) - \nabla h(x)^\top(z-x)$. We first link stationarity with gradient norms in the next lemma. 


\begin{lemma}
\label{lem:stationarity}
     Let $\alpha > 0$, and $0 < \gamma \leq \frac{1}{L}$. Let $G(x) := \|x -  \prox_{\gamma \Phi}(x)\|_1$ denote the stationarity gap.. Then for any $x \in \Delta^{|\calS|}$ such that for all $i \in [1, |\calS|],\; x_i \geq \alpha$, we have that
    \[
    -\langle A\br{z-x}, \nabla \Phi(Ax) \rangle \leq \br{\frac{6}{\alpha\gamma} + 2nmc_{\max}}G(x)
    \]
    for any $z \in \Delta^{|\calS|}$.
\end{lemma}
\begin{proof}
    Let $x' = \prox_{\gamma \Phi}(x)$. We know from optimality conditions applied to \eqref{eq:MD} that 
    \[
    A^\top \nabla \Phi(Ax') =  \frac{1}{\gamma}\bs{ \nabla h(x) - \nabla h(x')} + c\mathrm{1}= 0
    \]
    For any $z \in \Delta^{|\calS|}$, by Holder's inequality, we have
    \begin{equation}
    -\langle A\br{z-x}, \nabla \Phi(Ax) \leq \rangle \leq \frac{1}{\gamma} \innerprod{\nabla h(x') - \nabla h(x)}{z-x} + m\|\nabla \Phi(Ax) - \nabla \Phi(Ax')\|_\infty.
    \label{eq:holder}
    \end{equation}
    Now since $\forall i \in [1, |\calS|],\; x_i \geq \alpha$, we also have that $\forall i \in [1, |\calS|],\; x_i' \geq \alpha e^{-\gamma L}$. Consequently,
    \[
    |\nabla h(x)_i - \nabla h(x')_i| = |\log(x_i) - \log(x_i')| \leq \frac{1}{\alpha e^{-\gamma L}} |x_i - x_i'| \leq \frac{e^{\gamma L}G(x)}{\alpha}
    \]
    Plugging this in \eqref{eq:holder} and using the fact that $\gamma < \frac{1}{L}$ yields the result.
\end{proof}

\begin{lemma}[From stationarity to Nash] Let $\alpha >0$ and let $x \in \Delta^{|\calS|}$ such that $x_i > \alpha$ for all $i \in \{1, \dots, |\calS|\}$. If $x$ is $\epsilon$-stationary, i.e, $G(x) \leq \epsilon$, then
\[
c(x_i, x_{-i}) - \min_{\bar{x}_i} c(\bar{x}_i, x_{-i}) \leq \br{\frac{6}{\alpha\gamma} + 2nmc_{\max}} \epsilon .
\]
\end{lemma}

\begin{proof} By linearity we have that,
\[
\begin{aligned}
    c(x_i, x_{-i}) - \min_{\bar{x}_i} c(\bar{x}_i, x_{-i}) &= -\innerprod{A\br{\bar{x} - x}}{\nabla \Phi (Ax)}
\end{aligned}
\]
we conclude by invoking Lemma \ref{lem:stationarity}.
\end{proof}

With these lemmas in hand we proceed to proving that the iterates of Algorithm~\ref{alg:bandit-alg} attain a low average stationarity gap. We will follow the proof strategy used in 




